ML-Decoder: Scalable and Versatile Classification Head

In this paper, we introduce ML-Decoder, a new attention-based classification head. ML-Decoder predicts the existence of class labels via queries, and enables better utilization of spatial data compared to global average pooling. By redesigning the decoder architecture, and using a novel group-decoding scheme, ML-Decoder is highly efficient, and can scale well to thousands of classes. Compared to using a larger backbone, ML-Decoder consistently provides a better speed-accuracy trade-off. ML-Decoder is also versatile - it can be used as a drop-in replacement for various classification heads, and generalize to unseen classes when operated with word queries. Novel query augmentations further improve its generalization ability. Using ML-Decoder, we achieve state-of-the-art results on several classification tasks: on MS-COCO multi-label, we reach 91.4% mAP; on NUS-WIDE zero-shot, we reach 31.1% ZSL mAP; and on ImageNet single-label, we reach with vanilla ResNet50 backbone a new top score of 80.7%, without extra data or distillation. Public code is available at: https://github.com/Alibaba-MIIL/ML_Decoder

==> Tables/nus_comparison_avi.tex <==
\begin{table*}[t]
\centering
\caption{State-of-the-art comparison for ZSL and GZSL tasks on the NUS-WIDE and Open Images datasets. We report the results in terms of mAP, as well as precision (P), recall (R), and F1 score at $K{\in}\{3,5\}$ for NUS-WIDE and $K{\in}\{10,20\}$ for Open Images. Best results are in bold. }
\adjustbox{width=\linewidth}{
\begin{tabular}{ccccccccc|ccccccc} 
\toprule[0.15em]
\multirow{3}{*}{\textbf{ Method}} & \multirow{3}{*}{\textbf{Task }} & \multicolumn{7}{c}{\textbf{NUS-WIDE ( \#seen / \#unseen = 925/81) }} & \multicolumn{7}{c}{\textbf{Open-Images ( \#seen / \#unseen = 7186/400) }} \\
 &  & \multicolumn{3}{c}{\textbf{K = 3 }} & \multicolumn{3}{c}{\textbf{K = 5 }} & \multirow{2}{*}{\textbf{mAP }} & \multicolumn{3}{c}{\textbf{K = 10 }} & \multicolumn{3}{c}{\textbf{K = 20 }} & \multirow{2}{*}{\textbf{mAP }} \\
 &  & \textbf{P } & \textbf{R } & \textbf{F1 } & \textbf{P } & \textbf{R } & \textbf{F1 } &  & \textbf{P } & \textbf{R } & \textbf{F1 } & \textbf{P } & \textbf{R } & \textbf{F1 } &  \\ 
\toprule[0.15em]
\multirow{2}{*}{CONSE~\cite{norouzi2013zero}} & ZSL & 17.5 & 28.0 & 21.6 & 13.9 & 37.0 & 20.2 & 9.4 & 0.2 & 7.3 & 0.4 & 0.2 & 11.3 & 0.3 & 40.4 \\
 & GZSL & 11.5 & 5.1 & 7.0 & 9.6 & 7.1 & 8.1 & 2.1 & 2.4 & 2.8 & 2.6 & 1.7 & 3.9 & 2.4 & 43.5 \\ 
\cmidrule(lr){2-16}
\multirow{2}{*}{LabelEM~\cite{akata2015label}} & ZSL & 15.6 & 25.0 & 19.2 & 13.4 & 35.7 & 19.5 & 7.1 & 0.2 & 8.7 & 0.5 & 0.2 & 15.8 & 0.4 & 40.5 \\
 & GZSL & 15.5 & 6.8 & 9.5 & 13.4 & 9.8 & 11.3 & 2.2 & 4.8 & 5.6 & 5.2 & 3.7 & 8.5 & 5.1 & 45.2 \\ 
\cmidrule(lr){2-16}
\multirow{2}{*}{Fast0Tag~\cite{zhang2016fast}} & ZSL & 22.6 & 36.2 & 27.8 & 18.2 & 48.4 & 26.4 & 15.1 & 0.3 & 12.6 & 0.7 & 0.3 & 21.3 & 0.6 & 41.2 \\
 & GZSL & 18.8 & 8.3 & 11.5 & 15.9 & 11.7 & 13.5 & 3.7 & 14.8 & 17.3 & 16.0 & 9.3 & 21.5 & 12.9 & 45.2 \\ 
\cmidrule(lr){2-16}
\multirow{2}{*}{One Attention per Label~\cite{kim2018bilinear}} & ZS & 20.9 & 33.5 & 25.8 & 16.2 & 43.2 & 23.6 & 10.4 & - & - & - & - & - & - & - \\
 & GZSL & 17.9 & 7.9 & 10.9 & 15.6 & 11.5 & 13.2 & 3.7 & - & - & - & - & - & - & - \\ 
\cmidrule(lr){2-16}
\multirow{2}{*}{LESA (M=10)~\cite{huynh2020shared}} & ZSL & \textbf{25.7} & {41.1} & \textbf{31.6} & \textbf{19.7} & {52.5} & \textbf{28.7} & 19.4 & 0.7 & 25.6 & 1.4 & 0.5 & 37.4 & 1.0 & 41.7 \\
 & GZSL & 23.6 & 10.4 & 14.4 & 19.8 & 14.6 & 16.8 & 5.6 & 16.2 & 18.9 & 17.4 & 10.2 & 23.9 & 14.3 & 45.4 \\ 
 \cmidrule(lr){2-16}
  
 \multirow{2}{*}{AviBC et. al. (M=7)} & ZSL & {24.2}  & {\textbf{41.3}}  & {30.5}  & {18.8}  & {\textbf{53.4}}  & {27.8}  & {\textbf{25.9}}  & \textbf{{6.1}} & \textbf{{47.0}} & \textbf{{10.7}} & \textbf{{4.4}}  & \textbf{{68.1}} & \textbf{{8.3}} & \textbf{{62.9}} \\
 & GZSL & {\textbf{27.7}}  & {\textbf{13.9}}  & {\textbf{18.5}}  & {\textbf{23.0}}  & {\textbf{19.3}}  & {\textbf{21.0}}  & {\textbf{12.1}}  & \textbf{{35.3}} & \textbf{{40.8}} & {\textbf{37.8}} & \textbf{{23.6}} & {\textbf{54.5}} & {\textbf{32.9}} & {\textbf{75.3}} \\
  \cmidrule(lr){2-16}

\multirow{2}{*}{Ours} & ZSL & {24.2}  & {\textbf{41.3}}  & {30.5}  & {18.8}  & {\textbf{53.4}}  & {27.8}  & {\textbf{25.9}}  & \textbf{{6.1}} & \textbf{{47.0}} & \textbf{{10.7}} & \textbf{{4.4}}  & \textbf{{68.1}} & \textbf{{8.3}} & \textbf{{62.9}} \\
 & GZSL & {\textbf{27.7}}  & {\textbf{13.9}}  & {\textbf{18.5}}  & {\textbf{23.0}}  & {\textbf{19.3}}  & {\textbf{21.0}}  & {\textbf{12.1}}  & \textbf{{35.3}} & \textbf{{40.8}} & {\textbf{37.8}} & \textbf{{23.6}} & {\textbf{54.5}} & {\textbf{32.9}} & {\textbf{75.3}} \\
  \cmidrule(lr){2-16}
  
\bottomrule[0.1em]
\end{tabular}
}
\vspace{-0.15cm}
\label{tab:sota_nuswide_openimages}
\end{table*}


==> Tables/query_sampling_vs_full.tex <==
\begin{table*}[hbt!]
\centering
\begin{tabular}{c|c|c|c|c|c|c|c} 
\hline
\begin{tabular}[c]{@{}c@{}}Decoder \\Type\end{tabular} & \begin{tabular}[c]{@{}c@{}}Number of (train)\\Classes\end{tabular} & \begin{tabular}[c]{@{}c@{}}Number of \\Queries\end{tabular} & \begin{tabular}[c]{@{}c@{}}Flops \\{[}G]\end{tabular} & \begin{tabular}[c]{@{}c@{}}Rate \\{[}fps]\end{tabular} & \begin{tabular}[c]{@{}c@{}}Max \\batch size\end{tabular} & \begin{tabular}[c]{@{}c@{}}mAP \\{[}\%]\end{tabular} & \begin{tabular}[c]{@{}c@{}}F1(K=3) \\{[}\%]\end{tabular}  \\ 
\hline
None                                                   & 925                                                         & —                                                           & 5.7                                                   & ???                        & ???                                                       & ???                                                           & ???                                                  \\ 
\hline
FUll                                                   & 925                                                         & 925                                                          & ???                                                   & 354                       & 216                                                       & 28.4                                                           & 31.2                               \\ 
\hline
QS                                                  & 925                                                         & 500                                                          & ???                                                   & 615                          & 456                                                       & 29.0                                                           & 31.1                                   \\
QS                                                  & 925                                                         & 200                                                           & ???                                                   & ???                         & ???                                                   & 29.0                                                       & 31.3                                   \\
QS                                                  & 925                                                         & 50                                                           & ???                                                   & 612                         & 456                                                       & 28.4                                                             & 29.2                                   \\

\hline
\end{tabular}
\caption{\textbf{Comparison of NUS-WIDE ZS mAP scores for different query sampling (\textbf{QS}) schemes.} }
\label{Table:nus_qs_schems}
\end{table*}

==> Tables/single_label.tex <==
% \usepackage{caption}


\begin{table}[hbt!]
\centering
\begin{tabular}{c|c|c|c} 
\Xhline{3\arrayrulewidth}
\begin{tabular}[c]{@{}c@{}}Pooling\\Scheme\end{tabular} & Backbone & \begin{tabular}[c]{@{}c@{}}Top1 \\Acc. [\%]\end{tabular} & \begin{tabular}[c]{@{}c@{}}Flops\\{[}G]\end{tabular}  \\ 
\Xhline{3\arrayrulewidth}
GAP                                                     & ResNet50 & 79.7                                                     & 4.1                                                   \\ 
\hline
ML-Decoder                                              & ResNet50 & 83.3                                                     & 4.7                                                   \\
\hline
\end{tabular}
\caption{\textbf{ImageNet classification scores for different pooling schemes}. For ML-Decoder, we used group-decoding with 100 groups. Our training configuration is A2~\cite{wightman2021resnet}.}
\label{Table:single_label_results}
\end{table}

==> latex/related.tex <==
\label{related}
\subsection{(Generalized) Zero-Shot Learning}

==> latex/scheme_2.tex <==
% We will now focus on the task of multi-label ZSL.
% Using ML-Decoder for multi-label ZSL is straight-forward, and requires minimal architectural modifications. 
Next, we will discuss several key features of ML-Decoder which make it suitable for multi-label ZSL. In addition, we will present several modifications which we apply in the ZSL setting in order to improve generalizability.
%
We begin by presenting a version of ML-Decoder for ZSL with full-decoding (using one label per query, $K=N$).
% In the previous section we have presented ML-Decoder design for regular multi-label classification. We will now focus on the task of multi-label ZSL. We will discuss the the key features of our method which makes it generalizable to ZSL, and how we improve this generalizability with the introduction of a novel query-augmentation. In addition, we will discuss how we can apply the group-decoding scheme in the ZSL setting, to improve its scalability. 
% Using ML-Decoder for multi-label ZSL is straight-forward and requires minimal architectural modifications. In the ZSL setting, we will start by presenting a version of ML-Decoder without group-decoding. \\ %, and then show how we incorporate group-decoding
\vspace{-0.2cm}
\paragraph{NLP word embeddings:} The first modification related to ZSL is to use word embeddings extracted from a text model as the per-label input queries.  As discussed in  the previous section, the input queries can be either learnable or fixed. For ZSL we chose to use word embeddings as the fixed queries.
For each label $n$, an embedding vector $L_n$ is extracted using a language model. The set of the word-embedding vectors is used as $G_q$ in Eq.~\ref{eq:ML-decoder} (see also Figure ~\ref{fig:zsl_scheme}). 
% An embedding vector $N_i$ is extracted for the word associated with each label $i$, and the . 
This allows the semantic information captured by the word embeddings to propagate from the \emph{seen} (training) classes to the \emph{unseen} (test) classes during inference. 
%
\vspace{-0.15cm}
\paragraph{ML-Decoder features:} ML-Decoder is well suited for ZSL due to several favorable features. Firstly, its attention mechanism is based on dot-product similarity between vectors (Eq.~\ref{eq:Attention}). Since NLP word embeddings preserve this dot-product semantic similarity~\cite{goldberg2014word2vec}, the unseen labels are more likely to be matched with the most similar keys and values within the decoder. 
ML-Decoder allows a variable number of input queries, and is not sensitive to the order of queries. This is beneficial since in ZSL we perform training and testing on different sets of classes, and therefore different sets of queries. 
For ZSL we train exclusively on the seen labels, and perform inference on the unseen classes, while for Generalized ZSL (GZSL), we perform inference on the union of the unseen and seen sets of labels.
% Applying this feature to our advantage, we train using the training set classes exclusively, and perform inference with the same model using a different set of classes. For the task of Generalized Zero-Shot Learning (GZSL) we use the full set of labels (train and test labels) for inference, while for ZSL we exclusively use test set labels.\\
\vspace{-0.15cm}
\paragraph{Further modifications:} Another modification of ML-Decoder for the ZSL setting is using shared parameters for the learnable projection matrix of the group fully-connected layer (setting $W_k=W$ in Eq.~\ref{eq:group_fc}). By using a shared parameter matrix for all classes, we are able to transfer information from the seen to the unseen classes.

Group-decoding (with $K<N$) also requires modifications in order to work in the ZSL setting. In appendix~\ref{zsl_scalability} we thoroughly detail our variant of group-decoding for ZSL. 
% (see also the pseudo-code in appendix \ref{appendix:zsl_group_code}).
%
% In section~\ref{experiments} we will show how each of these modifications contribute to the final classification score. 
%
\vspace{-0.2cm}
\paragraph{Query-Augmentation} 
% \TBD{tal's note: currently the motivation for query augmentation is a bit thin. i suggest adding another line that states the analogy between regular image augmentations and query augmentations. usually only the image is the input, and that's what we augment, quite heavily, to prevent overfit, \textbf{encourage generalization} and get good results (auto-augment, cutout, mixup,..). now we have another type of input, queries, so it's logical and reasonable also to augment it\\}
ML-Decoder naturally extends to the task of ZSL. Yet, we want to apply dedicated training tricks that further improve the model's generalizability.
%
It is common practice in computer vision to apply augmentations on the input images to prevent overfitting, and improve generalizability to new unseen images. Similarly, we introduce novel \emph{query augmentations} to encourage generalization to unseen class queries.
% and to tackle the problem of over-fitting which plagues Zero-Shot learning techniques 
% ($W_i=W$ for all $i$, in equation~\ref{eq:fc_regular_decoder})
% $z_i\in \mathbb{R}^{d_h}$ (from eqn.~\ref{eq:regular_decoder})
% We can apply two types of augmentations on the input queries, which encourage the model to generalize to classes which were unseen during training
The first augmentation is \emph{random-query}, which adds additional random-valued queries to the set of input queries, and assigns a positive ground truth label signifying “random” for these added queries. The second augmentation is \emph{query-noise}, where we add each batch a small random noise to the input queries. See Figure~\ref{fig:query_aug} in the appendix for illustration of the augmentations. In  Section~\ref{sec:zsl_results} we will show that query augmentations encourage the model to recognize novel query vectors which it hasn’t encountered before, and improve ZSL scores. We also tried query-cutout augmentation, where random parts of the queries are deleted each batch. However, this technique was not beneficial in our experiments. 
% \begin{figure}[hbt!]
%     \centering
%     \includegraphics[width=0.48\textwidth]{pics/query_augmentation.pdf}
%     \caption{\textbf{Query augmentations} \emph{rand-query}: adding random queries which are assigned label "noise". \emph{additive noise}: adding random noise to the input queries.
%     % \emph{noise}: adding small gaussian noise to the queries.
%     }
%     \label{fig:query_aug}
%     \vspace{-0.15cm}
% \end{figure}
